The Complexity of Graph Exploration Games

Graph Exploration problems ask a searcher to explore an unknown environment. The environment is modeled as a graph, where the searcher needs to visit each vertex beginning at some vertex. Treasure Hunt problems are a variation of Graph Exploration, in which the searcher needs to find a hidden treasure, which is located at a designated vertex. Usually these problems are modeled as online problems, and any online algorithm performs poorly because it has too little knowledge about the instance to react adequately to the requests of the adversary. Thus, the impact of a priori knowledge is of interest. One form of a priori knowledge is an unlabeled map, which is an isomorphic copy of the graph. We analyze Graph Exploration and Treasure Hunt problems with an unlabeled map that is provided to the searcher. For this, we formulate decision variants of both problems by interpreting the online problems as a game between the online algorithm (the searcher) and the adversary. The map, however, is not controllable by the adversary. The question is whether the searcher is able to explore the graph completely or find the treasure for all possible decisions of the adversary. We analyze these games in multiple settings, with and without costs on the edges, on directed and undirected graphs and with different constraints (allowing multiple visits to vertices or edges) on the solution. We prove PSPACE-completeness for most of these games. Additionally, we analyze the complexity of related problems that have additional constraints on the solution.

==> src/path-relaxing-short.tex <==
% !TEX root=lipics-paper.tex
\subsection{Relaxing the Path Constraint}
\label{sec:trail}\label{sec:walk}
The goal of this subsection is to analyze all variants of online search sequence games based on s-t path.
The variants span over three dimensions: the constraint on the search sequence (path, trail, walk), a cost function on the edges (no costs or unit costs), the underlying graph (directed or undirected).

We begin with the easiest variant, the undirected walk without costs.
This problem degenerates to the \LSPACE-complete \textsc{Undirected s-t Connectivity} \cite{DBLP:journals/jacm/Reingold08} because if the vertices $s$ and $t$ are connected, the online algorithm can explore the complete graph and finally reach $t$.

All other variants are \PSPACE-complete.
We reuse the presented reduction from \qsatgame{} to \ostupg{} and extend it by using different techniques to derive the results for the other variants.
For the \ostutg{} without costs, we replace every vertex $p^i_j$ in the variable gadget with two vertices $p^i_j$ and $q^i_j$, connected by an edge $\{p^i_j, q^i_j\}$, with the sinks attached to $q^i_j$ instead of $p^i_j$.
The edges $\{u^i_3, p^i_1\}$, $\{u^i_4, p^i_j\}$ remain unchanged, for $j \in \{1, 2, 3, 4\}$.
The edges $\{p^i_j, p^i_{j+1}\}$ are replaced by $\{q^i_j, p^i_{j+1}\}$, for $j \in \{1, 2, 3\}$.
All remaining edges starting in $p^i_j$ start in $q^i_j$ instead, for $j \in \{1, 2, 3, 4\}$. 
This change prevents the algorithm from visiting $u^i_4$ and thus $u^i_5$ multiple times, such that $x_i$ cannot be set to both true and false.
Thus, the algorithm needs to travel along the zig-zag path over the $p^i_j$ and $q^i_j$.

From a slight modification of this reduction, we are also able to deduce the \PSPACE-completeness of \ostuwg{} with costs.
The problem is that the online algorithm is able to leave the sinks once they are visited and is potentially able to go along the colored edges from \Cref{st:fig:variable}.
Thus, we need to ensure that the algorithm receives large costs, whenever a sink is used.
For this, let $\ell$ be the length of the s-t path in the reduction.
We first duplicate all sinks by introducing $\ell$ additional sinks to all vertices that have a sink.
Secondly, we assign every edge costs of $1$.
Thus, if the algorithm tries to use a colored edge, the adversary can force it to visit all sinks before that.

\paragraph{Directed Graphs}
The results for the directed variants follow from the corresponding undirected variant.
For this, we modify the reduction such that the edges are directed in the direction of travel and exploration.
That is, all edges in \Cref{st:fig:variable} are mapped to arcs  that go from left to right.
The edge $\{u_2^i, u_3^i\}$ is mapped to two arcs $(u_2^i, u_3^i)$ and $(u_3^i, u_2^i)$ and the edges from $\{p_k^i, p_{k+1}^i\}$ are replaced by arcs $(p_k^i, p_{k+1}^i)$ for $k \in \{1,2,3\}$.
The clause gadgets are directed in the direction of travel as well.
The resulting graph is a directed acyclic graph up to the cycles induced by $(u_2^i, u_3^i)$ and $(u_3^i, u_2^i)$.
These cycles, however, are never a subwalk of the resulting walk because it is optimal to use exactly one of the arcs once.
Thus, every walk or trail in the graph is also a path because it is impossible to go back.



\paragraph{Overview}
All our results for online games based on $s$-$t$-connectivity problems are summarized in \Cref{path:tab:results}.
All \PSPACE-completeness results follow from the completeness of \ostuwg{} with costs, \ostutg{} without costs and \ostdwg{} without costs.

\begin{table}[t]
	\centering
	\begin{tabular}{ll|l|l}
		\multicolumn{2}{l|}{}                                    & no costs                                                              & unit costs                       \\ \hline
		\multicolumn{1}{l|}{\multirow{2}{*}{Path}}  & undirected & \multirow{2}{*}{\PSPACE-complete}                                      & \multirow{2}{*}{\PSPACE-complete} \\ \cline{2-2}
		\multicolumn{1}{l|}{}                       & directed   &                                                                       &                                  \\ \hline
		\multicolumn{1}{l|}{\multirow{2}{*}{Trail}} & undirected & \multirow{2}{*}{\PSPACE-complete}                                      & \multirow{2}{*}{\PSPACE-complete} \\ \cline{2-2}
		\multicolumn{1}{l|}{}                       & directed   &                                                                       &                                  \\ \hline
		\multicolumn{1}{l|}{\multirow{2}{*}{Walk}}  & undirected & \LSPACE-complete                                                            & \multirow{2}{*}{\PSPACE-complete} \\ \cline{2-3}
		\multicolumn{1}{l|}{}                       & directed   &  
		\PSPACE-complete&                                 
	\end{tabular}
	\caption{
		The complexity of online games based on $s$-$t$-connectivity problems.
	}
	\label{path:tab:results}
\end{table}


==> src/proofs/0proofTemplate.tex <==
% !TEX root=lipics-paper.tex


==> src/vertexOrderingProblems-short.tex <==
% !TEX root=lipics-paper.tex
\section{Hamiltonian Problems}
\label{sec:hampath}

The second class of problems are Hamiltonian problems, which can be interpreted as decision variants of Graph Exploration problems.
These problems ask for a search sequence visiting all vertices of the graph.
The corresponding cost variant is the \otsg{}.

For this class of problems, we are also able to construct reductions from \qsatgame{}.
However, we need to use other techniques due to the lack of sinks.
Sinks are not possible because the online algorithm has to visit all vertices and if a sink is introduced into the instance, the instance is a trivial NO-instance.
In order to circumvent this problem, the adversary needs to force the online algorithm to cut itself off by earlier visited vertices.

For the reduction, we reuse the reduction from \textsc{Satisfiability} to \textsc{Hamiltonian Path} by Arora and Barak \cite{DBLP:books/daglib/0023084}.
Again, we introduce additional edges to reveal the way through the gadgets such that the online algorithm is able to find a path satisfying the given \qsat{} formula.
With slight modifications, we can also apply these results to other variants of the problem.
In \Cref{ham:tab:results}, our results for online games based on Hamiltonian path problems are presented.
The fields with ? remain unanswered.


\begin{table}[t]
	\centering
	\begin{tabular}{ll|l|l}
		\multicolumn{2}{l|}{}                                    & no costs                                                              & unit costs                       \\ \hline
		\multicolumn{1}{l|}{\multirow{2}{*}{Path}}  & undirected & \multirow{2}{*}{\PSPACE-complete}                                      & \multirow{2}{*}{\PSPACE-complete} \\ \cline{2-2}
		\multicolumn{1}{l|}{}                       & directed   &                                                                       &                                  \\ \hline
		\multicolumn{1}{l|}{\multirow{2}{*}{Trail}} & undirected & \multirow{2}{*}{?}                                      & \multirow{2}{*}{\PSPACE-complete} \\ \cline{2-2}
		\multicolumn{1}{l|}{}                       & directed   &                                                                       &                                  \\ \hline
		\multicolumn{1}{l|}{\multirow{2}{*}{Walk}}  & undirected & \LSPACE-complete                                                            & \multirow{2}{*}{\PSPACE-complete} \\ \cline{2-3}
		\multicolumn{1}{l|}{}                       & directed   & 
		?&                                 
	\end{tabular}
	\caption{
		The complexity of different \ohpg\textsc{s}.
	}
	\label{ham:tab:results}
\end{table}

